AIDA: An Active Inference-based Design Agent for Audio Processing Algorithms

In this paper we present AIDA, which is an active inference-based agent that iteratively designs a personalized audio processing algorithm through situated interactions with a human client. The target application of AIDA is to propose on-the-spot the most interesting alternative values for the tuning parameters of a hearing aid (HA) algorithm, whenever a HA client is not satisfied with their HA performance. AIDA interprets searching for the "most interesting alternative" as an issue of optimal (acoustic) context-aware Bayesian trial design. In computational terms, AIDA is realized as an active inference-based agent with an Expected Free Energy criterion for trial design. This type of architecture is inspired by neuro-economic models on efficient (Bayesian) trial design in brains and implies that AIDA comprises generative probabilistic models for acoustic signals and user responses. We propose a novel generative model for acoustic signals as a sum of time-varying auto-regressive filters and a user response model based on a Gaussian Process Classifier. The full AIDA agent has been implemented in a factor graph for the generative model and all tasks (parameter learning, acoustic context classification, trial design, etc.) are realized by variational message passing on the factor graph. All verification and validation experiments and demonstrations are freely accessible at our GitHub repository.

==> 04-background.tex <==

\section{Optimal selection of parameter trials} \label{sec:efe}

The goal of proposing alternative HA tuning parameter settings (task 3) is to receive positive user responses in the future. Free energy minimization over desired future user responses can be achieved through a procedure called ``Expected Free Energy'' (EFE) minimization \citep{friston_active_2015,sajid_active_2020}. 

EFE as a trial selection criterion induces a natural trade-off between explorative (information seeking) and exploitative (reward seeking) behaviour. In the context of situated HA personalization, this is desirable because soliciting user feedback can be burdensome and invasive, as described in Section~\ref{sec:problem:AIDA}. From the agent's point of view, this means that striking a balance between gathering information about user preferences and satisfying learned preferences is vital. The EFE provides a way to tackle this trade-off, inspired by neuro-scientific evidence that brains operate under a similar protocol \citep{friston_active_2015,parr_uncertainty_2017}.

To arrive at the EFE formulation , we start by a generative model $p(r, v \mid \bm{u})$ for observations of user responses $r$, latent states $v$, and parameter trials $\bm{u} \in \mathcal{U}$, where $\mathcal{U}$ is a set of admissible trials. After $r$ has been observed, we can write down a variational free energy (VFE) functional
\begin{align}\label{eq:vfe_xz}
    F_{\bm{u}}[q] &= \mathbb{E}_{q(v \mid \bm{u})} \left[ \ln \frac{q(v\mid \bm{u})}{p(r,v\mid \bm{u})} \right] \,,
\end{align}
that scores the Kullback-Leibler divergence (a distance measure) between a variational distribution $q(v\mid \bm{u})$ and a generative model $p(r,v\mid \bm{u})$. 
Note that \eqref{eq:vfe_xz} is a \emph{functional} of the variational distribution $q(v\mid\bm{u})$ for a given trial $\bm{u}$. In order to select a new parameter trial, it is important that we to anticipate what the listener's future responses $r$ is going to be for that trial. This poses a problem for computing \eqref{eq:vfe_xz} since this requires user responses from the future which, by definition, have not been observed yet.
To address this problem, we can take the \emph{expectation} of the VFE with respect to future observations $r$ as  \eqref{eq:vfe_xz} as
\begin{subequations}\label{eq:efe}
\begin{align}
    G_{\bm{u}}[q]
    &= \mathbb{E}_{q(r\mid v, \bm{u})}\left[ F_{\bm{u}}[q]\right] \\
    &= \mathbb{E}_{q(r,v\mid \bm{u})} \left[ \ln \frac{q(v\mid \bm{u})}{p(r,v\mid \bm{u})} \right]\,,
\end{align}
\end{subequations}
which is known as the Expected Free Energy criterion for trials $\bm{u}$. We can decompose the EFE to reveal some desirable properties. Starting from \eqref{eq:efe} we can show that
\begin{align}
    G_{\bm{u}}[q]
    &\approx \underbrace{\mathbb{E}_{q(r \mid \bm{u})} \bigg[ \ln \frac{1}{p(r)} \bigg]}_{\text{Utility drive}}
    -\underbrace{\mathbb{E}_{q(r,v\mid \bm{u})} \bigg[ \ln \frac{q(v \mid \bm{u}, r)}{q(v \mid \bm{u})} \bigg]}_{\text{Information gain}}\,, \label{eq:efe_bound}
\end{align}
which balances an information gain term and versus a utility-driven term. A full derivation of \eqref{eq:efe_bound} is provided in Appendix \ref{appendix:efe_derivations}.

The utility drive pushes the agent towards matching predicted user responses $q(r \mid \bm{u})$ with a goal prior over \emph{desired} user responses $p(r)$. This goal prior allows encoding of beliefs about future observations that we wish to observe. Setting the goal prior to match positive user responses then drives the agent towards parameter settings that it believes make the user happy in the future.

The information gain term in \eqref{eq:efe_bound} drives agents that optimize the EFE to seek out responses that are maximally informative about latent states $v$. To see why this is so, we can rewrite the information gain term into two entropy terms  
\begin{equation}\label{eq:entropy_reduc}
\begin{split}
    \mathbb{E}_{q(r,v\mid \bm{u})} \bigg[ \ln \frac{q(v \mid \bm{u}, r)}{q(v \mid \bm{u})} \bigg]
    &= \mathrm{H}[v \mid \bm{u}] - \mathbb{E}_{q(r \mid \bm{u})}\bigg[ \mathrm{H}[v \mid \bm{u}, r] \bigg]\\
    &= \mathrm{H}[r \mid \bm{u}] - \mathbb{E}_{q(v \mid \bm{u})}\bigg[ \mathrm{H}[r \mid \bm{u}, v] \bigg]
    \end{split}
\end{equation}
where $\mathrm{H}[\cdot]$ denotes entropy. What \eqref{eq:entropy_reduc} shows is that we can view information gain as the expected reduction in posterior entropy over $v$ from receiving the observation $r$. Since we can think of entropy as a measure of uncertainty, the reduction in entropy quantifies how much information we expect to gain from a particular observation. Furthermore it is easy to verify that we can write the information gain in terms of both entropies over $r$ and $v$. We will make use of this fact later when deriving the expression for EFE used in AIDA.
Readers coming from a machine learning or information theory background may recognise the utility drive as a cross-entropy loss term and information gain as a mutual information term. Evaluating  $G_{\bm{u}}[q]$ as a function of $\bm{u}$ provides our method for action selection which we will detail in Section~\ref{sec:inference:agent}.

==> A3-model.tex <==
\section{Probabilistic model overview}\label{appendix:model}
This appendix gives a concise overview of the generative model of the acoustic model and AIDA. The prior distributions are uninformative unless stated otherwise in Section~\ref{sec:experiments}.
\subsection{Acoustic model}
\vspace{-50pt}
\begin{subequations}
    \begin{align*}
        \intertext{The observed signal $x_t$ is the sum of a speech and noise signal as}
        x_t &= s_t + n_t
        \intertext{The speech signal $s_t = \bm{e}_1^\intercal\bm{s}_t$ is modeled by a time-varying auto-regressive process as}
        \bm{s}_t &\sim \mathcal{N}\left(A(\bm{\theta}_t)\bm{s}_{t-1},\ V\left(\gamma\right)\right)
        \intertext{The auto-regressive coefficients of the speech signal are time-varying as}
        \bm{\theta}_t &\sim \mathcal{N}\left(\bm{\theta}_{t-1},\ \omega\mathrm{I}_{M}\right)
        \intertext{The noise signal $n_t = \bm{e}_1^\intercal\bm{n}_t$ is also modeled by an auto-regressive process}
        \bm{n}_t &\sim \mathcal{N}\left(A(\bm{\zeta}_k)\bm{n}_{t-1},\ V\left(\tau_k\right)\right) \qquad\qquad \text{for }t = t^-, t^-+1, \ldots, t^+
        \intertext{The parameters of the noise model depend on the context}
        \bm{\zeta}_k &\sim \prod_{l=1}^L \mathcal{N}\left(\bm{\mu}_{l}, \Sigma_{l}\right)^{c_{lk}} \\
        \tau_k &\sim \prod_{l=1}^L \Gamma\left(\alpha_{l}, \beta_{l}\right)^{c_{lk}} \\
        \intertext{The context $\bm{c}_k$ evolves over a different time scale indexed by $k$ as}
        \bm{c}_k &\sim \mathrm{Cat}(\mathrm{T}\bm{c}_{k-1})
        \intertext{The transition matrix of the context is modeled as}
        \mathrm{T}_{1:L,j} &\sim \mathrm{Dir}(\bm{\alpha}_j)
        \intertext{Finally, the output of the hearing aid algorithm $y_t$ is formed as the weighted sum of the speech and noise signals as}
        y_t &= u_{sk}s_t + u_{nk}n_t \qquad\qquad \text{for }t = t^-, t^-+1, \ldots, t^+
    \end{align*}
\end{subequations}

\subsection{AIDA's user response model}
\vspace{-30pt}
\begin{subequations}
    \begin{align*}
        \intertext{The user responses are modeled by a Bernoulli distribution containing a Gaussian cumulative probability distribution that enforces the output $v_k(\bm{u}_k$) to the allowed domain for the argument of the Bernoulli distribution}
        r_k &\sim \mathrm{Ber}(\Phi(v_k(\bm{u}_k))) \qquad\qquad \text{if } r_k \in\{0,1\}
        \intertext{$v_k(\bm{u}_k)$ encodes our beliefs about the user response function (evaluated at $\bm{u}_k$), modeled by a mixture of Gaussian processes as}
        v_k &\sim \prod_{l=1}^L\mathrm{GP}(m_l(\cdot),K_l(\cdot,\cdot))^{c_{lk}}
        \intertext{whose kernel function is defined as}
        K(\bm{u},\bm{u}^\prime) &= \sigma^2 \exp\left\{-\frac{\|\bm{u}-\bm{u}^\prime\|^2_2}{2l^2}\right\}
        \intertext{where $\sigma$ denotes noise and $l$ the length scale of the kernel.}
        %K_l(a,b) &= \sigma_l^2 \exp \left( -\frac{(a - b)^2}{2l_l^2} \right)
    \end{align*}
\end{subequations}
%The agent model is a standard Gaussian Process Classifier (GPC) with a squared exponential kernel. The GPC is given by 
%
%\begin{subequations}
%\begin{align*}
   
%   v &\sim \mathrm{GP}(m(\cdot),K(\cdot,\cdot)) \label{eq:model:GP}
% \end{align*}
% \end{subequations}
%
% where $\Phi(\cdot)$ denotes the Gaussian CDF. Without loss of generality, we can set the mean function of the GP to 0 \citep{rasmussen_gaussian_2006}. The kernel function $K(\cdot,\cdot)$ is given by
% \begin{align*}
%     K(a,b) &= \sigma^2 \exp \bigg( -\frac{(a - b)^2}{2l^2} \bigg)
% \end{align*}

%\bart{Below details should go in the experimental validation section}
%\mtk{Updated}

%For our experiments we initialised $\sigma = l = 0.5$ and performed updates using the LBFGS implementation of Optim.jl, v1.5.0 at every $5^th$ iteration. 
%User responses are sampled from a Bernoulli distribution with parameter $\theta_{user}$ computed as
%\begin{align*}
%    \theta_{user} &= \frac{2}{1 + \exp( \beta \sum_k  \frac{(\bm{u}_k - \bm{u}_k^*)^2}{\sigma_k} )}
%\end{align*}
%For our experiments we set 
%\begin{align*}
%    \bm{u}^* &= [0.8,0.2] \\
%    \sigma &= [1,1] \\
%    \beta &= 25 
%\end{align*}
\vspace{100pt}
\begin{table}[ht]
    \centering
    \caption{Summary of the notational conventions used throughout Section~\ref{sec:model} in this paper.}
    \label{tab:symbols-model}
    \begin{tabular}{c|c|p{13cm}}
        Notation & Definition & Explanation \\ \hline \hline
        $x_t$ & \eqref{eq:model:acoustic} & Observed signal at time index $t$. \\
        $y_t$ & \eqref{eq:model:HA-output} & Output of the hearing aid at time index $t$. \\
        $s_t$ & & Latent speech signal at time index $t$.\\
        $n_t$ & & Latent noise signal at time index $t$. \\
        $\bm{s}_t$ & \eqref{eq:model:acoustic:AR} & Vector with hidden states of the auto regressive model of the speech signal at time index $t$. \\
        $\bm{n}_t$ & \eqref{eq:model:acoustic-noise} & Vector with hidden states of the auto regressive model of the noise signal at time index $t$. \\
        $\bm{\theta}_t$ & \eqref{eq:model:acoustic:coefs} & Vector of auto regressive coefficients of the speech signal at time index $t$. \\
        $\omega$ & & Covariance matrix scaling of the dynamics of the auto regressive coefficients of the speech signal. \\
        $\mathrm{I}_M$ & & Identity matrix of size $(M\times M)$. \\
        $M$ & & Auto regressive order of the speech signal. \\
        $N$ & & Auto regressive order of the noise signal. \\
        $W$ & & Sampling ratio between $t$ and $k$. \\
        $A(\theta)$ & \eqref{eq:model:ARmatrix} & State space transition matrix of an auto regressive process with coefficients $\bm{\theta}$. \\
        $\gamma$ & & Process noise precision of the auto regressive model for the speech signal. \\
        $V(\gamma)$ & & Covariance matrix of the auto regressive model for the speech signal, containing only zeros except for the first element, which is $1/\gamma$. \\
        $\bm{e}_i$ & & Appropriately sized cartesian standard unit vector containing only zeros, except for the $i^\text{th}$ entry, which is 1. \\
        $\bm{0}$ & & Appropriately sized vector of zeros. \\
        $\mathcal{N}(\mu, \Sigma)$ & & Normal distribution with mean $\mu$ and covariance matrix $\Sigma$. \\
        $\Gamma(\alpha, \beta)$ & & Gamma distribution with shape and rate parameters $\alpha$ and $\beta$, respectively. \\
        $\bm{\zeta}_k$ & \eqref{eq:model:zeta} & Vector of auto-regressive coefficients of the noise signal at context time scale index $k$.\\
        $\tau_k$ & \eqref{eq:model:tau} & Process noise precision of the auto regressive model of the noise signal at context time scale index $k$. \\
        $L$ & & Number of contexts. \\
        $\bm{c}_k$ & \eqref{eq:model:context-dynamics} & The context at context time scale $k$, containing a 1-of-$L$ binary vector with elements $c_{lk}\in\{0,1\}$. \\
        $\bm{\pi}$ & & Vector of event probabilities. \\
        $\mathrm{T}$ & \eqref{eq:model:context-transition} & Transition matrix representing the discrete context dynamics. \\
        $\bm{\alpha}_j$ & & Concentration parameters for the prior over the $j^\text{th}$ column of $T$. \\
        $u_{sk}$ & & Gain of the speech signal at context time index $k$. \\
        $u_{nk}$ & & Gain of the noise signal at context time index $k$. \\
        $\bm{u}_k$ & & Vector of tuning parameters at context time index $k$ defined as $[u_{sk}, u_{nk}]^\intercal$. \\
        $v_k(\cdot)$ & \eqref{eq:model:GP-1} & Latent function drawn from a mixture of GPs. \\
        $r_k$ & \eqref{eq:sigmoid-user-response-1}& Binary user response at time index $k$. \\
        $\Phi(\cdot)$ & & Standard Gaussian cumulative distribution function. \\
        $m_l(\cdot)$ & & Mean function of the $l^\text{th}$ GP. \\
        $K_l(\cdot, \cdot)$ & & Kernel function of the $l^\text{th}$ GP.
    \end{tabular}
\end{table}
